Estimating County-Level COVID-19 Exponential Growth Rates Using Generalized Random Forests

Rapid and accurate detection of community outbreaks is critical to address the threat of resurgent waves of COVID-19. A practical challenge in outbreak detection is balancing accuracy vs. speed. In particular, while estimation accuracy improves with longer fitting windows, speed degrades. This paper presents a machine learning framework to balance this tradeoff using generalized random forests (GRF), and applies it to detect county level COVID-19 outbreaks. This algorithm chooses an adaptive fitting window size for each county based on relevant features affecting the disease spread, such as changes in social distancing policies. Experiment results show that our method outperforms any non-adaptive window size choices in 7-day ahead COVID-19 outbreak case number predictions.

==> Backup.tex <==

\iffalse
\subsection{Formal Assumptions}
Due to the nature of the data available to us being at varying levels of granularity both along the time and geographical axes, 
we have to make assumptions regarding the causal nature of features and how they relate to the dependent variable and the estimated rate of change.\\

\noindent \textbf{A1:} Counties inherit the features of their states
    
\begin{align}
    \forall t \geq 0, \forall S \subset C, \forall c \in S: X_{t,S} = X \Rightarrow X_{t,c} = X
\end{align}

While this assumption seems needlessly obvious for some features like laws and policies like shutting down of schools, availability of paid sick leave etc. due to the geopolitical structure of the US, some features need not necessarily exhibit such property, such as the state level test positivity rate amongst racial groups, which is a weighted average of data not available to us.\\  

\noindent \textbf{A2:} Time points inherit features indexed by an interval that contains them 
\begin{align*}
    \forall G \subset \{0,1,2,\dotsc,t_{\max}\}, \forall t \in G, \forall c \in C:\\ 
    X_{G,c} = X \Rightarrow X_{t,c} = X  
\end{align*}

Again, this assumption trivially holds for boolean type data, e.g. if there was a ban on social gatherings in the month of June, we can reason that every day in the month of June has such a realization of the feature, but this need not apply for aggregates such as a monthly average of some feature.\\

\noindent \textbf{A3:} Lipschitz feature signal

\begin{align*}
    X_{i} \mapsto r_{i}\\
    \exists K \in \mathbb{R}^{+}\backslash\{0\}: d_{r}(\hat{r}_{1},\hat{r}_{2}) &\leq K d_{X}(X_1 , X_2) 
\end{align*}

This is a more explicit paraphrasing of the "Lipschitz $x$-signal" assumption in \cite{athey2019generalized} which states that the effect of what we wish to estimate (rate of change of case numbers for our work) should vary Lipschitz continuously with respect to the feature space.
In layman terms, features that are close enough should output similar predictions.
While this is part of a larger set of assumptions for their methodology which we will adapt for our framework,
it is also the key motivation behind our feature engineering which we will present later.\\

\noindent \textbf{A4: } Dependent variable data is not right censored \\

While the reported case numbers for some counties are left censored, as we only obtain  data once there is at least one case occurrence, we assume that once a county has appeared in the data, 
it is continuously tracked. 
This is a relatively benign assumption given the nature of the dataset we are working with.  
\fi

\section{Application to COVID-19 Dataset}
\subsection{Description of Datasets}

\subsection{Backtest and Validation}

\begin{table}[hbtp]
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:example-booktabs}%
  {\caption{RMSE and MAPE Averages Post 30th April 2020}}%
  {\begin{tabular}{lll}
  \toprule
  \bfseries Model & \bfseries RMSE & \bfseries MAPE\\
  \midrule
  OLS.wsize=16 & 0.2325 & 0.0510 \\
  OLS.wsize=8 & 0.1924  & 0.04276 \\
  OLS.wsize=4 &  0.1618 & 0.0362\\
  OLS.wsize=2 & 0.1444 & 0.0324\\
  \textbf{GRF.wsize=2} & \textbf{0.1379} & \textbf{0.0309}\\
  \bottomrule
  \end{tabular}}
\end{table}

==> Estimating the Exponential Growth Rate of COVID-19 Using Generalized Random Forest (ML4H)/Backup.tex <==

\iffalse
\subsection{Formal Assumptions}
Due to the nature of the data available to us being at varying levels of granularity both along the time and geographical axes, 
we have to make assumptions regarding the causal nature of features and how they relate to the dependent variable and the estimated rate of change.\\

\noindent \textbf{A1:} Counties inherit the features of their states
    
\begin{align}
    \forall t \geq 0, \forall S \subset C, \forall c \in S: X_{t,S} = X \Rightarrow X_{t,c} = X
\end{align}

While this assumption seems needlessly obvious for some features like laws and policies like shutting down of schools, availability of paid sick leave etc. due to the geopolitical structure of the US, some features need not necessarily exhibit such property, such as the state level test positivity rate amongst racial groups, which is a weighted average of data not available to us.\\  

\noindent \textbf{A2:} Time points inherit features indexed by an interval that contains them 
\begin{align*}
    \forall G \subset \{0,1,2,\dotsc,t_{\max}\}, \forall t \in G, \forall c \in C:\\ 
    X_{G,c} = X \Rightarrow X_{t,c} = X  
\end{align*}

Again, this assumption trivially holds for boolean type data, e.g. if there was a ban on social gatherings in the month of June, we can reason that every day in the month of June has such a realization of the feature, but this need not apply for aggregates such as a monthly average of some feature.\\

\noindent \textbf{A3:} Lipschitz feature signal

\begin{align*}
    X_{i} \mapsto r_{i}\\
    \exists K \in \mathbb{R}^{+}\backslash\{0\}: d_{r}(\hat{r}_{1},\hat{r}_{2}) &\leq K d_{X}(X_1 , X_2) 
\end{align*}

This is a more explicit paraphrasing of the "Lipschitz $x$-signal" assumption in \cite{athey2019generalized} which states that the effect of what we wish to estimate (rate of change of case numbers for our work) should vary Lipschitz continuously with respect to the feature space.
In layman terms, features that are close enough should output similar predictions.
While this is part of a larger set of assumptions for their methodology which we will adapt for our framework,
it is also the key motivation behind our feature engineering which we will present later.\\

\noindent \textbf{A4: } Dependent variable data is not right censored \\

While the reported case numbers for some counties are left censored, as we only obtain  data once there is at least one case occurrence, we assume that once a county has appeared in the data, 
it is continuously tracked. 
This is a relatively benign assumption given the nature of the dataset we are working with.  
\fi

\section{Application to COVID-19 Dataset}
\subsection{Description of Datasets}

\subsection{Backtest and Validation}

\begin{table}[hbtp]
 % The first argument is the label.
 % The caption goes in the second argument, and the table contents
 % go in the third argument.
\floatconts
  {tab:example-booktabs}%
  {\caption{RMSE and MAPE Averages Post 30th April 2020}}%
  {\begin{tabular}{lll}
  \toprule
  \bfseries Model & \bfseries RMSE & \bfseries MAPE\\
  \midrule
  OLS.wsize=16 & 0.2325 & 0.0510 \\
  OLS.wsize=8 & 0.1924  & 0.04276 \\
  OLS.wsize=4 &  0.1618 & 0.0362\\
  OLS.wsize=2 & 0.1444 & 0.0324\\
  \textbf{GRF.wsize=2} & \textbf{0.1379} & \textbf{0.0309}\\
  \bottomrule
  \end{tabular}}
\end{table}

==> Estimating the Exponential Growth Rate of COVID-19 Using Generalized Random Forest (ML4H)/images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}


==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}

